Deep Learning to Estimate Permeability using Geophysical Data

Time-lapse electrical resistivity tomography (ERT) is a popular geophysical method to estimate three-dimensional (3D) permeability fields from electrical potential difference measurements. Traditional inversion and data assimilation methods are used to ingest this ERT data into hydrogeophysical models to estimate permeability. Due to ill-posedness and the curse of dimensionality, existing inversion strategies provide poor estimates and low resolution of the 3D permeability field. Recent advances in deep learning provide us with powerful algorithms to overcome this challenge. This paper presents a deep learning (DL) framework to estimate the 3D subsurface permeability from time-lapse ERT data. To test the feasibility of the proposed framework, we train DL-enabled inverse models on simulation data. Subsurface process models based on hydrogeophysics are used to generate this synthetic data for deep learning analyses. Results show that proposed weak supervised learning can capture salient spatial features in the 3D permeability field. Quantitatively, the average mean squared error (in terms of the natural log) on the strongly labeled training, validation, and test datasets is less than 0.5. The R2-score (global metric) is greater than 0.75, and the percent error in each cell (local metric) is less than 10%. Finally, an added benefit in terms of computational cost is that the proposed DL-based inverse model is at least O(104) times faster than running a forward model. Note that traditional inversion may require multiple forward model simulations (e.g., in the order of 10 to 1000), which are very expensive. This computational savings (O(105) - O(107)) makes the proposed DL-based inverse model attractive for subsurface imaging and real-time ERT monitoring applications due to fast and yet reasonably accurate estimations of the permeability field.

==> Sections/HGP_DL_Figures.tex <==
%****************************************;
%                                        ;
%  NAME                                  ;
%    HGP_DL_Figures.tex                  ;
%                                        ;
%  WRITTEN BY                            ;
%    Maruti Kumar Mudunuru               ;
%                                        ;
%****************************************;

%-------------------------------------------------;
%  Figure-1: Permeability field (Train/Val/Test)  ;
%-------------------------------------------------;
\begin{figure}
  \centering
  \subfigure[Training realization]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Perm_Ground_Truth/1_train_gt_24.png}}
  %
  \subfigure[Training realization]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Perm_Ground_Truth/1_train_gt_25.png}}
  %
  \subfigure[Training realization]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Perm_Ground_Truth/1_train_gt_26.png}}
  %
  \subfigure[Validation realization]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Perm_Ground_Truth/87_val_gt_24.png}}
  %
  \subfigure[Validation realization]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Perm_Ground_Truth/87_val_gt_25.png}}
  %
  \subfigure[Validation realization]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Perm_Ground_Truth/87_val_gt_26.png}}
  %
    \subfigure[Test realization]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Perm_Ground_Truth/75_test_gt_24.png}}
  %
  \subfigure[Test realization]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Perm_Ground_Truth/75_test_gt_25.png}}
  %
  \subfigure[Test realization]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Perm_Ground_Truth/75_test_gt_26.png}}
  %
  \caption{\textbf{Multiple realizations of 3D permeability field (synthetic data) for hydrogeophysics simulations:}~This figure show samples of the permeability realizations generated for developing hydrogeophysics simulation data.
  The top, middle, and bottom figures show 2D slices of the 3D permeability field at different depths.
  They also show the spatial patterns of permeability field that DL-enabled inverse models need to capture across training, validation, and testing sets.
  \label{Fig:Perm_Realz_Data}}
\end{figure}

%---------------------------------------------------;
%  Figure-2: ERT simulation and observational data  ;
%---------------------------------------------------;
\begin{figure}
  \centering
  \subfigure[Raw data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_rawmeas_1.png}}
  %
  \subfigure[Raw data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_rawmeas_26.png}}
  %
  \subfigure[Raw data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_rawmeas_34.png}}
  %
  \subfigure[Raw data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_rawmeas_48.png}}
  %
  \subfigure[Raw data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_rawmeas_1033.png}}
  %
  \subfigure[Raw data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_rawmeas_1041.png}}
  %
  \subfigure[Normalized data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_normmeas_1.png}}
  %
  \subfigure[Normalized data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_normmeas_26.png}}
  %
  \subfigure[Normalized data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_normmeas_34.png}}
  %
  \subfigure[Normalized data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_normmeas_48.png}}
  %
    \subfigure[Normalized data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_normmeas_1033.png}}
  %
  \subfigure[Normalized data]
    {\includegraphics[width = 0.325\textwidth]
    {Figures/Pots_Sim_vs_Obs/Sim_normmeas_1041.png}}
  %
  \caption{\textbf{Simulations vs. observational time-lapse ERT data:}~This figure shows samples of raw and normalized transfer resistance among 40,466 measurements.
  Each of the blue and red lines corresponds to raw and normalized simulation data for 28 different times.
  The black line represents the observational data.
  Note that there are 200 blue/red lines for each measurement.  
  From this figure, it is evident that the observational data is contained within the normalized synthetic data.
  \label{Fig:ERT_Sim_Obs_Data}}
\end{figure}

%------------------------------------;
%  Figure-3: Deep learning workflow  ;
%------------------------------------;
\begin{figure}
  \centering
    \includegraphics[width = 1.05\textwidth]{Figures/DL_Workflow/DL_Workflow_v1.pdf}
  \caption{\textbf{Proposed DL methodology:}~A pictorial description of the proposed workflow to develop DL-enabled inverse models.
  The top figure shows the process of mapping the electrical potential field to the permeability field.
  PCA is used to perform dimensionality reduction to encode and decode transfer resistance and 3D permeability data.
  The bottom figure shows a fully connected DNN architecture to map the encoded potential to the encoded permeability field.
  Hyperparameter tuning (e.g., number of neurons in each layer, learning rate) is performed to identify tuned DNN architectures.
  The predicted principal components are decoded using the permeability PCA estimator to obtain the predicted 3D permeability field.
  \label{Fig:DL_Workflow_Architecture}}
\end{figure}

%------------------------------------------------------------;
%  Figure-4: PCA variance distribution (Perm and Potential)  ;
%------------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[Potential field:~EVR vs. principal components]
    {\includegraphics[width = 0.475\textwidth]{Figures/PCA_EVS/PCA_Potential_EVS.png}}
    %
    \subfigure[Permeability field:~EVR vs. principal components]
    {\includegraphics[width = 0.475\textwidth]{Figures/PCA_EVS/PCA_Perm_EVS.png}}
  %
  \caption{\textbf{PCA-based dimensionality reduction:}~This figure shows the distribution of variance ratio for all the principal components determined using the PCA estimators of permeability and electrical potential fields.
  The left and right figures show the variances for time-lapse ERT data and 3D permeability field, respectively. 
  The PCA estimators are developed on the 180 realizations of training data with 0.99 variances.
  This PCA training resulted in 91 and 160 principal components that represent potential and permeability fields, respectively.
  Each bar in these figures represents a principal component, which explains the variance in the simulation data.
  The extracted components are then used to transform the validation and test datasets.
  \label{Fig:PCA_Variance_eEeP}}
\end{figure}

%--------------------------------------------------------------------------------;
%  Figure-5: PCA reconstruction and associated percent errors in each grid cell  ;
%--------------------------------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[Training:~Ground truth vs. prediction]
    {\includegraphics[width = 0.32\textwidth]{Figures/PCA_IT_Errors/PCA_train_perm_error_unscaled.png}}
    %
    \subfigure[Validation:~Ground truth vs. prediction]
    {\includegraphics[width = 0.32\textwidth]{Figures/PCA_IT_Errors/PCA_val_perm_error_unscaled.png}}
    %
    \subfigure[Testing:~Ground truth vs. prediction]
    {\includegraphics[width = 0.32\textwidth]{Figures/PCA_IT_Errors/PCA_test_perm_error_unscaled.png}}
    %
    \subfigure[Training:~PCA reconstruction error]
    {\includegraphics[width = 0.325\textwidth]{Figures/PCA_IT_Errors/1_train_err_24.png}}
    %
    \subfigure[Validation:~PCA reconstruction error]
    {\includegraphics[width = 0.325\textwidth]{Figures/PCA_IT_Errors/87_val_err_24.png}}
    %
    \subfigure[Testing:~PCA reconstruction error]
    {\includegraphics[width = 0.325\textwidth]{Figures/PCA_IT_Errors/75_test_err_24.png}}
    %
    \subfigure[KDE vs. PCA reconstruction error]
    {\includegraphics[width = 0.375\textwidth]{Figures/PCA_IT_Errors/KDE_PCAIT1_Error.pdf}}
    %
  \caption{\textbf{PCA reconstruction and associated percent errors:}~This figure shows the permeability PCA estimator predictions and its errors on training, validation, and test datasets.
  The top figure shows one-to-one plots of PCA estimator predictions (values in $\ln[k(\mathbf{x})]$) with the ground truth for all the realizations in each set.
  To be specific, each blue dot in (a), (b), and (c) represents a permeability value in a 3D grid cell.
  The middle figures show spatial patterns of reconstruction errors (values in percentage) for 2D slices shown in Fig.~\ref{Fig:Perm_Realz_Data}(a), (d), and (g).
  The bottom figure shows the KDE as a function of percent errors in each grid cell for all the training, validation, and test realizations.
  From spatial plots and KDE figure, it is evident that the error in each cell is less than 10\%.
  \label{Fig:PCA_Reconstruction_Errors}}
\end{figure}

%-------------------------------------------------------------------------;
%  Figure-6: Loss for all 15 random seeds (mixup and pre-computed mixup)  ;
%-------------------------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[No mixup]
    {\includegraphics[width = 0.465\textwidth]{Figures/Loss_Plots/Loss_Train_Val_Allseeds_NoMixup.pdf}}
    %
    \subfigure[Pre-computed mixup after PCA]
    {\includegraphics[width = 0.465\textwidth]{Figures/Loss_Plots/Loss_Train_Val_Allseeds_PreMixup.pdf}}
    %
  \caption{\textbf{Loss metrics for 15 different best inverse models:}~This figure shows the overall training and validation loss of tuned DL-enabled inverse models for 15 different random seeds.
  The DNN architectures are tuned using strong (no mixup) and weak labels (without mixup).
  Based on the validation loss, it is evident that mixup training has slightly better generalization than no mixup.
  The number of epochs needed to reduced the loss for DL models trained on pre-computed mixup samples is considerably lower than no mixup. 
  This shows that weakly labeled data slightly helps to reduce over-fitting.
  However, we can see that the DL-enabled inverse models still over-fits the mixup data for more significant epochs (see the figure with epochs greater than 100).
  \label{Fig:Loss_Function_No_Precomp_Mixup}}
\end{figure}

%-------------------------------------------------------------;
%  Figure-11: One-to-One to plots of PCA and Perm components  ;
%-------------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[No mixup:~Training]
    {\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_IT_train_All_PCA_Comps_NoMixup.png}}
    %
    \subfigure[No mixup:~Validation]
    {\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_IT_val_All_PCA_Comps_NoMixup.png}}
    %
    \subfigure[No mixup:~Testing]
    {\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_IT_test_All_PCA_Comps_NoMixup.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Training]{\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_IT_train_All_PCA_Comps_PreMixup.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Validation]
    {\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_IT_val_All_PCA_Comps_PreMixup.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Testing]
    {\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_IT_test_All_PCA_Comps_PreMixup.png}}
    %
    \subfigure[No mixup:~Training]
    {\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_Perm_train_gt_All_Realz_NoMixup.png}}
    %
    \subfigure[No mixup:~Validation]
    {\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_Perm_val_gt_All_Realz_NoMixup.png}}
    %
    \subfigure[No mixup:~Testing]
    {\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_Perm_test_gt_All_Realz_NoMixup.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Training]
    {\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_Perm_train_gt_All_Realz_PreMixup.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Validation]
    {\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_Perm_val_gt_All_Realz_PreMixup.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Testing]
    {\includegraphics[width = 0.31\textwidth]{Figures/One_to_One_PCA_Plots/0_Perm_test_gt_All_Realz_PreMixup.png}}
    %
  \caption{\textbf{Ground truth vs. Prediction (PCA components and permeability):}~This figure shows one-to-one plots of a tuned DL-enabled inverse model (based on random seed = 0) for encoded and decoded 3D permeability.
  The top and middle figures show the PCA components predictions based on the tuned DNN architecture with and without mixup.
  Each blue dot represents an encoded permeability field.
  The lower set of figures show the predictions of decoded permeability field with and without mixup.
  These predictions are obtained by utilizing the trained PCA estimator on the DL predicted principal components.
  Each blue dot represents a permeability value in a grid cell.
  The permeability predictions based on DL-enabled inverse models trained using mixup samples seem to have slightly higher permeability values than no mixup.
  \label{Fig:True_vs_Pred_PermandPCA}}
\end{figure}

%----------------------------------------------------------;
%  Figure-8: Spatial plots of ground truth vs. prediction  ;
%----------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[No mixup:~Training prediction]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_NoMixup/1_train_pred_24.png}}
    %
    \subfigure[No mixup:~Validation prediction]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_NoMixup/87_val_pred_24.png}}
    %
    \subfigure[No mixup:~Testing prediction]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_NoMixup/75_test_pred_24.png}}
    %
    \subfigure[No mixup:~Training percent errors]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_NoMixup/1_train_err_24.png}}
    %
    \subfigure[No mixup:~Validation percent errors]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_NoMixup/87_val_err_24.png}}
    %
    \subfigure[No mixup:~Testing percent errors]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_NoMixup/75_test_err_24.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Training prediction]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_PreMixup/1_train_pred_24.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Validation prediction]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_PreMixup/87_val_pred_24.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Testing prediction]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_PreMixup/75_test_pred_24.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Training percent errors]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_PreMixup/1_train_err_24.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Validation percent errors]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_PreMixup/87_val_err_24.png}}
    %
    \subfigure[Pre-computed mixup after PCA:~Testing percent errors]
    {\includegraphics[width = 0.325\textwidth]{Figures/Spatial_Predictions_and_Errors_PreMixup/75_test_err_24.png}}
    %
  \caption{\textbf{Spatial prediction and associated percent errors with and without mixup:}~This figure shows the DL-enabled inverse models (based on random seed = 0) predictions and spatial distribution of percent errors.
  The top and middle figures show the DL model predictions and associated errors without mixup, while the lower figures show pre-computed mixup after PCA. 
  The corresponding ground truth for these predictions is shown in Fig.~\ref{Fig:Perm_Realz_Data}(a), (d), and (g).
  From the percent error 2D slices, it is evident that DL models trained using mixup data perform slightly better than without mixup.
  This is because mixup-trained DL models can better predict high permeability cells than models trained without mixup.
  \label{Fig:TrainValTest_Pred_Error}}
\end{figure}

%--------------------------------------------------------;
%  Figure-9: Distribution of R2-score and SSIM metrics  ;
%--------------------------------------------------------;
\begin{figure}
  \centering
    \subfigure[$R^2$-score]
    {\includegraphics[width = 0.485\textwidth]{Figures/Spatial_Predictions_and_Errors_NoMixup/KDE_Depth_R2.pdf}}
    %
    \subfigure[SSIM]
    {\includegraphics[width = 0.485\textwidth]{Figures/Spatial_Predictions_and_Errors_NoMixup/KDE_Depth_SSIM.pdf}}
    %
    \subfigure[Percent error in each grid cell]
    {\includegraphics[width = 0.485\textwidth]{Figures/Spatial_Predictions_and_Errors_NoMixup/KDE_percent_error.pdf}}
    %
  \caption{\textbf{Distribution of $R^2$-score, SSIM metric, and percent errors for with and without mixup:}~These figures compares the Kernel density estimates of all the 15 different tuned model trained with and without mixup.
  Metrics based on DL model predictions are evaluated at depths between 100m to 105m, the zone of interest.
  This zone is between the lowest and highest groundwater levels.
  The top left and right figures show the $R^2$-score and SSIM metric values, while the bottom figure shows the percent error in each cell.
  From $R^2$-score, quantitatively, it is evident that DL model predictions can capture the overall trends in the 3D permeability field.
  Qualitatively, it is clear that the percent errors in each cell are less than 10\%, and kernel density is concentrated primarily with 3\%.
  However, the SSIM score reveals reduced performance in capturing local patterns, which shows that over-fitting is still prevalent.
  In all these scenarios, the mixup trained model performs slightly better than no mixup.
  \label{Fig:TrainValTest_R2_SSIM}}
\end{figure}
